Implicit Neural Deformation for Sparse-View Face Reconstruction

In this work, we present a new method for 3D face reconstruction from sparse-view RGB images. Unlike previous methods which are built upon 3D morphable models (3DMMs) with limited details, we leverage an implicit representation to encode rich geometric features. Our overall pipeline consists of two major components, including a geometry network, which learns a deformable neural signed distance function (SDF) as the 3D face representation, and a rendering network, which learns to render on-surface points of the neural SDF to match the input images via self-supervised optimization. To handle in-the-wild sparse-view input of the same target with different expressions at test time, we propose residual latent code to effectively expand the shape space of the learned implicit face representation as well as a novel view-switch loss to enforce consistency among different views. Our experimental results on several benchmark datasets demonstrate that our approach outperforms alternative baselines and achieves superior face reconstruction results compared to state-of-the-art methods.

==> figs/fig_colorbar_stir.tex <==
\begin{figure*}%[t]
\centering
\begin{minipage}{0.48\linewidth}
\subfigure{\label{fig:colorbar_stir_sub1}
\includegraphics[width=\linewidth]{figures/colorbar_err/s18_v0_arrange1.pdf}}%s32_v0e50_arrange1

\vspace{-0.3cm}
\subfigure{\label{fig:colorbar_stir_sub3}
 \includegraphics[width=\linewidth]{figures/colorbar_err/s18_v1_arrange1_v1.pdf}}
\end{minipage}
\begin{minipage}{0.48\linewidth}
\subfigure{\label{fig:colorbar_stir_sub2}
\includegraphics[width=\linewidth]{figures/colorbar_err/s32_v0e50_arrange1_x.pdf}}%\vspace{-0.2cm}

\vspace{-0.3cm}
\subfigure{\label{fig:colorbar_stir_sub4}
\includegraphics[width=\linewidth]{figures/colorbar_err/s32_v1e20_arrange1_v1.pdf}}%\vspace{-0.15cm}
\end{minipage}
\caption{Geometry error maps on the Stirling$\slash$ESRC test set for different methods (\ie, DFNRMVS \cite{bai20dfnrmvs} and ours). The inputs are two-view images of an identity with two different expressions. In each triplet, the first column is the one of the two-view inputs, the second column is the geometry error map of DFNRMVS \cite{bai20dfnrmvs}, and the third column is our geometry error map.}
\label{fig:colorbar_stir}
\end{figure*}




==> figs/fig_details_bosp.tex <==
\begin{figure*}%[t]
\centering
\subfloat[eyelids]{
\label{Fig.sub.1}
\includegraphics[width=0.48\textwidth]{figures/s341_leye_patch.pdf}}
\subfloat[wrinkles]{
\label{Fig.sub.2}
\includegraphics[width=0.48\textwidth]{figures/reye_patch.pdf}}
\vspace{-3pt}
\caption{Qualitative comparison of local regions with DFNRMVS \cite{bai20dfnrmvs} on the Bosphorus dataset \cite{savran2008bosphorus}. In each triplet, the left column is the input, the second column is the 3D reconstruction of DFNRMVS \cite{bai20dfnrmvs}, and the last column is our reconstruction results.}
\label{fig:details_bosp}
\end{figure*}


==> figs/fig_rebuttal_deca_stir.tex <==
\newcommand\galleryfigurewidth{0.32}
\begin{figure}%[t]
\centering
% \subfloat[Instance 1]
{\begin{minipage}{0.92\linewidth}
\includegraphics[width=\galleryfigurewidth\linewidth]{figures/gallery_deca_stiresrc/s18/v0_orgimg_224.jpg}
\includegraphics[width=\galleryfigurewidth\linewidth]{figures/gallery_deca_stiresrc/s18/F1013_H1_0.jpg}
\includegraphics[width=\galleryfigurewidth\linewidth]{figures/gallery_deca_stiresrc/s18/v0_pred_vrts_render_224.jpg}

\includegraphics[width=\galleryfigurewidth\linewidth]{figures/gallery_deca_stiresrc/s19/v0_orgimg_224.jpg}
\includegraphics[width=\galleryfigurewidth\linewidth]{figures/gallery_deca_stiresrc/s19/F1046_S_0.jpg}
\includegraphics[width=\galleryfigurewidth\linewidth]{figures/gallery_deca_stiresrc/s19/v0_pred_vrts_render_224.jpg}
\end{minipage}
\hspace{-21pt}
\begin{minipage}{\galleryfigurewidth\linewidth}
    \centering
    \figtext{Input}
\end{minipage}
\begin{minipage}{\galleryfigurewidth\linewidth}
    \centering
    \figtext{\cite{feng2021learning}}
\end{minipage}
\begin{minipage}{\galleryfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}}
\vspace{-9pt}
\caption{\footnotesize Qualitative comparison with \cite{feng2021learning} on the Stirling$\slash$ESRC test set.
}
\label{fig:result_gallery_stiresrc_deca}
\end{figure}


==> figs/fig_supp_teaser_qualitative.tex <==
\newcommand\suppw{0.24}
\begin{figure*}%[t]
\centering
\subfloat[View 1]{\begin{minipage}{0.495\linewidth}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s1v0_orgimg.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s1v0_dfnpred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s1v0_ourspred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s1v0_predimg.png}

\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s2v0_orgimg.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s2v0_dfnpred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s2v0_ourspred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s2v0_predimg.png}

\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s3v0_orgimg.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s3v0_dfnpred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s3v0_ourspred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s3v0_predimg.png}

\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s4v0_orgimg.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s4v0_dfnpred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s4v0_ourspred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s4v0_predimg.png}
%
\hspace{-15pt}

\begin{minipage}{\suppw\linewidth}
    \centering
    \figtext{Input}
\end{minipage}
\begin{minipage}{\suppw\linewidth}
    \centering
    \figtext{DFNRMVS}
\end{minipage}
\begin{minipage}{\suppw\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\suppw\linewidth}
    \centering
    \figtext{Our Rendering}
\end{minipage}
\end{minipage}}
%
\subfloat[View 2]{\begin{minipage}{0.495\linewidth}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s1v1_orgimg.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s1v1_dfnpred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s1v1_ourspred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s1v1_predimg.png}

\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s2v1_orgimg.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s2v1_dfnpred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s2v1_ourspred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s2v1_predimg.png}

\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s3v1_orgimg.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s3v1_dfnpred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s3v1_ourspred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s3v0_predimg.png}

\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s4v1_orgimg.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s4v1_dfnpred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s4v1_ourspred.png}
\includegraphics[width=\suppw\linewidth]{figures/supp/inthewild/s4v1_predimg.png}
%
\hspace{-15pt}

\begin{minipage}{\suppw\linewidth}
    \centering
    \figtext{Input}
\end{minipage}
\begin{minipage}{\suppw\linewidth}
    \centering
    \figtext{DFNRMVS}
\end{minipage}
\begin{minipage}{\suppw\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\suppw\linewidth}
    \centering
    \figtext{Our rendering}
\end{minipage}
\end{minipage}}

\vspace{-7pt}
\caption{Qualitative comparison with DFNRMVS \cite{bai20dfnrmvs} for two-view input. Each row presents the inputs (\ie, view1, and view2) and corresponding results of one identity. In each quadruple, the first column is the one of the two input views, the second column is the reconstruction result of DRNRMVS \cite{bai20dfnrmvs}, the third column is our reconstructed mesh, and the last column is our rendering result.}
\label{fig:supp_teaser_qualitative}
\end{figure*}
% -----------------------------------


==> tables/tab_params.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{@{\extracolsep{\fill}} l | c |  c | c | c }
\hline
Method &  Ours  & \cite{bai20dfnrmvs} & \cite{bai2021riggable} & \cite{feng2021learning} \\
\hline
\# of params & 4.99M & 83.21M & 54.69M & 53.35M\\
\hline
\end{tabular}
\end{adjustbox}
%\vspace{-14pt}
\caption{\footnotesize Comparison of numbers of network parameters.}
\label{Table:Rebuttal_params}
\end{table}

